Permutohedral complexes and rational curves with cyclic action

We define a moduli space of rational curves with finite-order automorphism and weighted orbits, and we prove that the combinatorics of its boundary strata are encoded by a particular polytopal complex that also captures the algebraic structure of a complex reflection group acting on the moduli space. This generalizes the situation for Losev-Manin's moduli space of curves (whose boundary strata are encoded by the permutohedron and related to the symmetric group) as well as the situation for Batyrev-Blume's moduli space of curves with involution, and it extends that work beyond the toric context.

==> figures/delta32.tex <==
%% Creator: Inkscape inkscape 0.92.1, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'qqqq.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{320.64581924bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
      \begin{figure}[h!]
  \begin{picture}(1,1)%\begin{picture}(1,1.0166914)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{figures/delta32pdf.pdf}%
    \put(0.5,0.45){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\footnotesize{$S(3,2)$}}}%
    
    \put(0.76,0.60){\color[rgb]{1,0,0}\makebox(0,0)[lb]{\tiny{$y^0$}}}%
    \put(0.73,0.56){\color[rgb]{1,0,0}\makebox(0,0)[lb]{\tiny{$z^0_1$}}}%
    \put(0.86,0.56){\color[rgb]{1,0,0}\makebox(0,0)[lb]
    {\footnotesize{$\langle s_0 \rangle \begin{pmatrix}0 & 1 \\1 & 0 \end{pmatrix}$}}}%
    
    \put(0.78,0.45){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$y^0$}}}%
    \put(0.75,0.41){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$z^0_1$}}}%
    \put(0.72,0.41){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$z^0_2$}}}%
    \put(0.88,0.41){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\footnotesize{$\begin{pmatrix}0 & 1 \\1 & 0 \end{pmatrix}$}}}%
    
    \put(0.67,0.19){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$y^0$}}}%
    \put(0.64,0.15){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$z^0_2$}}}%
    \put(0.61,0.15){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$z^0_1$}}}%
    \put(0.77,0.15){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\footnotesize{$\begin{pmatrix}1 &0  \\0 &1 \end{pmatrix}$}}}%
    
    \put(0.51,0.16){\color[rgb]{0,0,1}\makebox(0,0)[lb]{\tiny{$y^0$}}}%
    \put(0.48,0.12){\color[rgb]{0,0,1}\makebox(0,0)[lb]{\tiny{$z^0_2$}}}%
    \put(0.48,0.03){\color[rgb]{0,0,1}\makebox(0,0)[lb]{\footnotesize{$\langle s_0 \rangle \begin{pmatrix}1 &0  \\0 &1 \end{pmatrix}$}}}%
    
    
    \put(0.34,0.06){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$y^0$}}}%
    \put(0.31,0.02){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$z^0_2$}}}%
    \put(0.28,0.02){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$z^1_1$}}}%
    \put(0.08,0.05){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\footnotesize{$\begin{pmatrix}\zeta^2 &0  \\0 &1 \end{pmatrix}$}}}%
    
    
    \put(0.77,0.79){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$y^0$}}}%
    \put(0.74,0.75){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$z^0_1$}}}%
    \put(0.71,0.75){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$z^1_2$}}}%
    \put(0.87,0.75){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\footnotesize{$\begin{pmatrix}0 & \zeta^2  \\ 1 & 0 \end{pmatrix}$}}}%
    
    
    \put(0.53,0.65){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$y^0$}}}%
    \put(0.51,0.605){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$z^0_1$}}}%
    \put(0.48,0.605){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\tiny{$z^2_2$}}}%
    \put(0.30,0.63){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\footnotesize{$\begin{pmatrix}0 & \zeta  \\1 & 0 \end{pmatrix}$}}}%
    
    \put(0.75,0.30){\color[rgb]{0,0.54117647,0}\makebox(0,0)[lb]{\tiny{$y^0$}}}%
    \put(0.72,0.33){\color[rgb]{0,0.54117647,0}\makebox(0,0)[lb]{\tiny{$z^0_1$}}}%
    \put(0.72,0.26){\color[rgb]{0,0.54117647,0}\makebox(0,0)[lb]{\tiny{$z^0_2$}}}%
    \put(0.85,0.26){\color[rgb]{0,0.54117647,0}\makebox(0,0)[lb]{\footnotesize{$\langle s_1 \rangle \begin{pmatrix}1 &0  \\0 &1 \end{pmatrix}$}}}%
      \end{picture}%
        \caption{A projection of the polytope $\Delta^3_2$, with some $\Delta$-faces labeled by both the boundary strata in $\L^3_2$ and by the corresponding $\T$-cosets in $S(3,2)$.}
   \label{fig:Delta32example}
   \end{figure}
\endgroup%

